Examining subgrid models of supermassive black holes in cosmological simulation

While supermassive black holes (SMBHs) play an important role in galaxy and cluster evolution, at present they can only be included in large-scale cosmological simulation via subgrid techniques. However, these subgrid models have not been studied in a systematic fashion. Using a newly-developed fast, parallel spherical overdensity halo finder built into the simulation code FLASH, we perform a suite of dark matter-only cosmological simulations to study the effects of subgrid model choice on relations between SMBH mass and dark matter halo mass and velocity dispersion. We examine three aspects of SMBH subgrid models: the choice of initial black hole seed mass, the test for merging two black holes, and the frequency of applying the subgrid model. We also examine the role that merging can play in determining the relations, ignoring the complicating effects of SMBH-driven accretion and feedback. We find that the choice of subgrid model can dramatically affect the black hole merger rate, the cosmic SMBH mass density, and the low-redshift relations to halo properties. We also find that it is possible to reproduce observations of the low-redshift relations without accretion and feedback, depending on the choice of subgrid model.

==> tab_mhalo_all.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
 Model  & con & con & con & con & m-s & m-s & m-s & m-s\\
\hline


==> tab_msigma_all.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
 Model  & con & con & con & con & m-s & m-s & m-s & m-s\\
\hline
con & -- & -- & -- & -- &  0.00 &  0.00 &  0.00 &  0.00\\
con & -- & -- & -- & -- &  0.00 &  0.00 &  0.00 &  0.00\\
con & -- & -- & -- & -- &  0.00 &  0.00 &  0.00 &  0.00\\
con & -- & -- & -- & -- &  0.00 &  0.00 &  0.00 &  0.00\\
m-s &  0.00 &  0.00 &  0.00 &  0.00 & -- & -- & -- & --\\
m-s &  0.00 &  0.00 &  0.00 &  0.00 & --m-sm-s &  0.00 &  0.00\hline
\end{tabular}

